Best arm identification in multi-armed bandits with delayed feedback

We propose a generalization of the best arm identification problem in stochastic multi-armed bandits (MAB) to the setting where every pull of an arm is associated with delayed feedback. The delay in feedback increases the effective sample complexity of standard algorithms, but can be offset if we have access to partial feedback received before a pull is completed. We propose a general framework to model the relationship between partial and delayed feedback, and as a special case we introduce efficient algorithms for settings where the partial feedback are biased or unbiased estimators of the delayed feedback. Additionally, we propose a novel extension of the algorithms to the parallel MAB setting where an agent can control a batch of arms. Our experiments in real-world settings, involving policy search and hyperparameter optimization in computational sustainability domains for fast charging of batteries and wildlife corridor construction, demonstrate that exploiting the structure of partial feedback can lead to significant improvements over baselines in both sequential and parallel MAB.

==> fixed_budget.tex <==
\section{The fixed budget setting}
Given a fixed time budget $T_{\max}$, an agent in this setting seeks to minimize the misidentification probability of the top-$k$ arms i.e.,
$Pr(A \neq \{1,2,\ldots,k\})$ for an accepted set of arms $A$. In particular, we consider the Successive Accepts and Rejects (SAR) algorithm that divides the total budget $T_{\max}$ into $n-1$ phases~\citep{bubeck2013multiple}. Similar to the racing procedures for the fixed confidence setting, it maintains disjoint sets of accepted arms $A$, rejected arms $R$, and surviving arms $S$ initialized to the full set of $n$ arms. During every phase $p$, we pull each surviving arm $t_p - t_{p-1}$ times, where $t_0=0$,
\begin{align*}
t_p &= \left\lceil \frac{1}{\overline{\log} n}\frac{T_{\max}-n}{n+1-p}\right\rceil
\end{align*}
for all $p \in \{1,2,\ldots,n-1\}$and $\overline{\log} n = \frac{1}{2}+\sum_{i=2}^n \frac{1}{i}$. Every phase eliminates an arm from the surviving set into either the accept or reject set, both initialized to be empty. If $\{\widehat{\mu}_i^s\}_{i=1}^{\vert S \vert}$ denotes the sorted (descending order) empirical means of the surviving arms, the eliminated arm corresponds to the one with the highest empirical gap defined below, 
\[
    \Delta_i^{<k'>} := 
\begin{cases}
    \widehat{\mu}_i^s -\widehat{\mu}_{k'+1}^s,& \text{if } i \leq k'\\
    \widehat{\mu}_{k'}^s - \widehat{\mu}_i^s,              & \text{otherwise}
\end{cases}
\] 
where $k'$ is the number of arms that remain to be accepted, i.e., $k'=k-\vert A \vert$. Note that the algorithm can exit early if $k'=0$ at the beginning of any phase and never takes a total budget more than $T_{\max}$ before termination. Using the above algorithm, \citet{bubeck2013multiple} showed that the misidentification probability can be upper-bounded as,
\begin{align*}
Pr(A \neq \{1,2,\ldots,k\}) \leq 2n^2 \exp\left(-\frac{T_{\max}-n}{8  \overline{\log}n H_2^{<k>}}\right)
\end{align*}
where the complexity measure $H_2^{<k>}=\max_{i=1,2,\ldots,n}i(\Delta_{i}^{<k>})^{-2}$.

In situations involving delayed feedback, the delays associated with the outcomes of any arm pull need to be accounted for in the alloted budget. To avoid pathological scenarios, we assume that no delay exceeds $D_{\max}$. We now propose algorithms based on SAR for the full and noisy delayed feedback settings.

\subsection{Full delayed feedback}
A naive extension of SAR to the full delayed feedback setting would involve splitting $T_{max}$ into $n-1$ phases as before and pulling each arm $\lfloor (t_p- t_{p-1}) / D_{\max}\rfloor $ times during phase $p$, 
% where,
% \begin{align*}
% t_p^d &= \left\lceil \frac{D_{\max}^{-1}}{\overline{\log} n}\frac{T_{\max}-n}{n+1-p}\right\rceil
% \end{align*}
until the budget for this phase  gets exhausted and an arm is eliminated. This procedure could however be wasteful since it assumes a worst case scenario where every arm pull has a delay of $D_{\max}$. In practice, a phase can get over much before the allocated time budget since the delays are stochastic. 

To account for the variability in delayed feedbacks, we propose an adaptive budget allocation algorithm, SARFullDF. Similar to vanilla SAR, SARFullDF operates in $n-1$ phases. At any given phase $p$, we pull each arm $t_p$ - $t_{p-1}$ times where 
\begin{align*}
t_p=\lfloor \left\lceil (T_{avail}^{<p>}-n_p)/(n_p\overline{\log} n_p)\right\rceil / D_{\max}\rfloor \quad \text{for } p=\{1,\ldots,n-1\}
\end{align*}
$t_0=0$, $T_{avail}^{<1>}=T_{\max}$, and $n_1=n$. If $T_{c}^{<p>}$ denotes the time consumed by the algorithm in the current phase, we reevaluate the number of pulls per arm for the next phase after making the following updates to the problem parameters.
\begin{align*}
T_{avail}^{<p+1>} \leftarrow T_{avail}^{<p>} -T_{c}^{<p>}, \,\,\,\,
n_{p+1} \leftarrow n_p - 1, \,\,\,\,
k' \leftarrow k - \vert A \vert
\end{align*}
Note that the accepted, rejected, and surviving arm sets are carried over from the previous phase. The criteria for elimination based on empirical gaps is same as SAR. We now provide a proof for the correctness of SARFullDF below.
\begin{lemma}
The SARFullDF algorithm terminates returning a set of $k$ accepted arms in no more than $T_{\max}$ steps.
\end{lemma}
\begin{proof}
We will prove the lemma in two parts. First, we will prove that the set of accepted arms contains exactly $k$ arms when the algorithm terminates. Finally, we will prove that the algorithm requires no more than $T_{\max}$ steps.

Since the algorithm runs in $n-1$ phases and every phase eliminates one arm, every arm will be assigned to the set of accepted or rejected arms by the end of $n-1$ phases. Using the fact that the number of elements in $A$ and $k'$ are constrained to sum to $k$ and $k'\leq \vert S \vert$ for any phase, we note that by the end of $n-1$ phases, $k'=0$ (since $\vert S \vert=0$) and hence, $\vert A\vert=k$. 

In phase $p$, we pull $n_p$ arms $t_p-t_{p-1}$ times where the delay of the $j$-th pull of arm $i$ in phase $p$ is given by $d_{p, i,j}$
such that the total budget consumed is given by,
\begin{align*}
\sum_{p=1}^{n-1}\sum_{i=1}^{n_p}\sum_{j=1}^{t_p-t_{p-1}}d_{p,i,j} &\leq \sum_{p=1}^{n-1}n_p (t_p -t_{p-1}) D_{\max} \leq \sum_{p=1}^{n-1}t_p D_{\max}\\
&\leq \sum_{p=1}^{n-1} \left\lfloor(T_{avail}^{<p>}-n_p)/(n_p\overline{\log} n_p)\right\rfloor \leq \sum_{p=1}^{n-1} \left\lfloor T_{\max}/n_p\overline{\log} n_p\right\rfloor \\
&\leq T_{\max}
\end{align*}
\end{proof}

The misindentification probability of SARFullDF can similarly be bounded as proved below.
\begin{lemma}

\end{lemma}

Misidentification of top-$k$ arms in SAR can arise due to acceptance of a sub-optimal arm (or rejection of an optimal arm) in any of the $n-1$ phases. Within any phase, pulling an arm has the effect of tightening the gap between the empirical mean and the true mean. Using noisy partial feedbacks, it is possible to design alternate estimators for the empirical mean that are within the same or tighter upper bounds on the distance from the true mean as naive empirical estimators from the full delayed feedback settings. These alternate estimators can be computed using only the partial feedbacks   We consider both cases of unbiased and biased partial feedbacks.

\subsection{Unbiased noisy partial feedback}

\begin{proposition}

\end{proposition}
reach the desired confidence for the surviving arms in a phase of SAR without having to wait for the pulls to actually finish.
\subsection{Biased noisy partial feedback}

